The Generalized Lasso for Sub-gaussian Measurements with Dithered Quantization

In the problem of structured signal recovery from high-dimensional linear observations, it is commonly assumed that full-precision measurements are available. Under this assumption, the recovery performance of the popular Generalized Lasso (G-Lasso) is by now well-established. In this paper, we extend these types of results to the practically relevant settings with quantized measurements. We study two extremes of the quantization schemes, namely, uniform and one-bit quantization; the former imposes no limit on the number of quantization bits, while the second only allows for one bit. In the presence of a uniform dithering signal and when measurement vectors are sub-gaussian, we show that the same algorithm (i.e., the G-Lasso) has favorable recovery guarantees for both uniform and one-bit quantization schemes. Our theoretical results, shed light on the appropriate choice of the range of values of the dithering signal and accurately capture the error dependence on the problem parameters. For example, our error analysis shows that the G-Lasso with one-bit uniformly dithered measurements leads to only a logarithmic rate loss compared to the full-precision measurements.

==> misc_submission.tex <==
\section{Miscellaneous}
\label{sec:misc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}\label{lem:key_uniform}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $\tau$ be a random variable distributed according to ${\rm Unif}\big(-\frac{\Delta}{2}, \frac{\Delta}{2}\big]$. Then for a fixed $x \in \R$, we have 
\begin{align}
\label{eq:xtau}
\mathbb{E}_{\tau}\Delta\Big(\Big\lfloor\frac{x + \tau}{\Delta}\Big\rfloor + \frac{1}{2} \Big) = x.
\end{align}
\end{lem}
\begin{proof}
Without loss of generality, we assume that $\Delta = 1$. 
%We want to show that 
%\begin{align}
%\mathbb{E}_{\tau}\Big(\floor{x + \tau}+ \frac{1}{2}\Big) = x, 
%\end{align}
%where $\tau \sim {\rm Unif}\Big(-\frac{1}{2}, \frac{1}{2}\Big]$. 
Note that depending on whether $0 \leq x - \floor{x} < \frac{1}{2}$ or $\frac{1}{2} \leq x - \floor{x} \leq 1$, we have
\begin{align}
\label{eq:xtau_1}
\floor{x + \tau} = \begin{cases}
\floor{x} - 1 & \text{if}~\tau \in \big(-\frac{1}{2}, \floor{x} - x\big),\\
\floor{x}  & \text{otherwise.}
\end{cases}
\end{align}
or 
\begin{align}
\label{eq:xtau_2}
\floor{x + \tau} = \begin{cases}
\floor{x} + 1 & \text{if}~\tau \in \big(\floor{x} +1 - x, \frac{1}{2}\big],\\
\floor{x}  & \text{otherwise.}
\end{cases}
\end{align}
respectively. We establish \eqref{eq:xtau} assuming that  $0 \leq x - \floor{x} < \frac{1}{2}$. The proof for the remaining case follows using the similar steps. Note that
\begin{align}
\mathbb{E}_{\tau}\Big(\floor{x + \tau}+ \frac{1}{2}\Big) &= \int_{-\frac{1}{2}}^{\frac{1}{2}} \floor{x + \tau} d\tau + \frac{1}{2} \nonumber \\ 
& \overset{(i)}{=}  \int_{-\frac{1}{2}}^{\frac{1}{2}} \floor{x} d\tau - \int_{-\frac{1}{2}}^{\floor{x} - x} d\tau  + \frac{1}{2} \nonumber \\
& = \floor{x} - \big(\floor{x} - x + \frac{1}{2}\big) + \frac{1}{2} = x,
\end{align}
where $(i)$ follows from \eqref{eq:xtau_1}.
\end{proof}

%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
\begin{lem}[Max of sub-exponential vector]\label{lem:max_exp}
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
Let $\ab=(a_1,a_2,\ldots,a_n)^T$ be an L-sub-gaussian random vector in $\R^n$. Then, 
\bea
\E\max_{i\in[n]} a_i^2 \leq C\,L^2\,\log{n}.
\eea
\end{lem}
\begin{proof}
First, note that each coordinate $a_i,i\in[n]$, is sub-gaussian with norm $\psin{a_i}\leq \max_{\ub\in\Sc^{n-1}}\psin{\ub^T\ab} = L$. Therefore, $a_i^2$ are sub-exponential with sub-exponential norm $\psinn{a_i}\leq L^2$ \cite[Lem.~2.7.6]{VerBook}. Thus, for some universal constants $c,C'>0$ and for all $0<\theta\leq \frac{c}{L^2}$, we have that~\cite[Lem.~5.15]{vershynin2010introduction}
\bea\nn
\E e^{\theta a_i^2} \leq e^{C'\theta^2L^4}.
\eea
Using this and the standard trick to bound the maximum of $n$ random variables, for all $0<\theta\leq \frac{c}{L^2}$, we have that 
\bea\nn
\E\max_{i\in[n]} a_i^2 \leq \frac{1}{\theta}\log\sum_{i\in [n]}\E e^{\theta a_i^2} \leq \frac{\log{n}}{\theta} + C'L^4\,\theta.
\eea
We may now choose (say) $\theta=c'/L^2$ to conclude with the desired.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{propo}[Rademacher comparison principle; Eqn.~(4.20) in \cite{ledoux}]\label{thm:contraction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $f~:~\R \to \R$ be a convex and increasing function. For $i \in [m]$, let $\phi_i : \R \to \R$ be a Lipschitz function with Lipschitz constant $\rho$, i.e., 
$
| \phi_i(x) - \phi_i(x')| \leq \rho |x - x'|,
$
such that $\phi_i(0) = 0$. Then, for any $\Sc \subseteq \R^m$, we have 
\begin{align}
\mathbb{E}f\Big(\sup_{\mathbf{t} = (t_1,\ldots, t_m) \in \Sc} \sum_{i = 1}^{m} \varepsilon_i \phi_i(t_i)\Big)  \leq \mathbb{E} f \Big( \rho \cdot \sup_{\mathbf{t} \in \Sc} \sum_{i = 1}^{m}\varepsilon_i t_i \Big),
\end{align}
where $\{\varepsilon_i\}_{i \in [m]}$ denote $m$ i.i.d. Rademacher random variables.
\end{propo}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background on $\gamma$-functionals}\label{sec:gamma}
For a set $\Tc$, we say that a sequence $\{\Ac_{n}\}$ of partitions of $\Tc$ is {\em increasing} if every set of $\Ac_{n+1}$ is contained in a set of $\Ac_n$. 
\begin{defn}[{Admissible sequence}]
Given a set $\Tc$, an admissible sequence is an increasing sequence $\{\Ac_n\}$ of partitions of $\Tc$ such that ${\rm card}(\Ac_n) \leq N_n {:= 2^{2^n}}$.
\end{defn}

\noindent Given a partition $\Ac_n$ of $\Tc$ and $\tb \in \Tc$, we use $A_n(\tb)$ to denote the set in $\Ac_n$ that contains $\tb$. With this notation in place, we now define a useful geometric quantity for the metric space $(\Tc, d)$. 
\begin{defn}
Given $\alpha > 0$ and a metric space $(\Tc, d)$, we define
\begin{align}
\label{eq:gamma_def}
\gamma_{\alpha}(\Tc, d) = \inf \sup_{\tb} \sum_{n \geq 0} 2^{n/\alpha}\Delta(A_n(\tb)),
\end{align}
where $\Delta(A_n(\tb))$ denotes the diameter of the set $A_n(\tb)$. The infimum in \eqref{eq:gamma_def} is taken over all admissible sequences.
\end{defn}

%In \cite[Theorem~1.2.7]{Tal}, Talagrand establish the following result.
\begin{propo}[{\cite[Thm.~1.2.7]{Tal}}]
\label{prop:Tal_Bern}
For a set $\Tc$ with two distances $d_1$ and $d_2$, consider a symmetric process $\{X_{\tb}\}_{\tb \in \Tc}$ such that $\E X_{\tb} = 0$ and $\forall~\s, \tb \in \Tc,~\forall~u > 0$,
\begin{align}\label{eq:Tal_Bern_1}
\Pro\left(\left\vert X_{\s} - X_{\tb}\right\vert \geq u\right) \leq 2\exp\left(-c\,\min\Big(\frac{u^2}{d_2(\s,\tb)^2}, \frac{u}{d_1(\s,\tb)}\Big)\right).
\end{align}
Then, for some universal constant $C>0$
\begin{align}\label{eq:Tal_Bern_2}
%\E\sup_{\s, \tb \in \Tc} \left\vert X_{\s} - X_{\tb}\right\vert
\E\sup_{\s \in \Tc}  X_{\s} \leq C\cdot\big(\gamma_1(\Tc, d_1) + \gamma_2(\Tc, d_2)\big).
\end{align}
\end{propo}
\begin{proof}
By \cite[Thm.~1.2.7]{Tal} the bound in \eqref{eq:Tal_Bern_2} holds for $\E\sup_{\s, \tb \in \Tc} \left\vert X_{\s} - X_{\tb}\right\vert$. However, for a symmetric process $X_\s$ it holds that $\E\sup_{\s, \tb \in \Tc} \left\vert X_{\s} - X_{\tb}\right\vert = 2\,\E\sup_{\s \in \Tc}  X_{\s}$; see \cite[Lem.~1.2.8]{Tal}.
\end{proof}


\begin{propo}[{ \cite[Thm.~2.6.2]{Tal}}]\label{prop:T_decom}
Consider a countable set $\Tc \subset \R^n$ such that $S= \gamma_2(\Tc, \ell_2) < \infty$. Then, for every number $\theta > 0$, there is a decomposition $\Tc \subset \Tc_1 + \Tc_2$ such that 
\begin{align}
\gamma_{2}(\Tc_1, \ell_2) \leq CS;~~\gamma_{1}(\Tc_1, \ell_{\infty}) \leq CS\theta \nn\\
\gamma_{2}(\Tc_2, \ell_2) \leq CS;~~\Tc_2 \subset \frac{CS}{\theta}\Bc_1. \nn
\end{align}
where $\Bc_1$ denotes the unit $\ell_1$-ball in $\R^n$ and $C>0$ denotes an absolute constant (that might be changing between the different four statements).
%Here, $\ell_1, d_2,$ and $d_{\infty}$ denote the distances induced by the norms $\|\cdot\|_1, \|\cdot\|_2,$ and $\|\cdot\|_{\infty}$, respectively.
\end{propo}

The following useful lemma is a simple corollary of Proposition \ref{prop:T_decom}. For a process that satisfies \eqref{eq:Tal_Bern_2} with $d_2$, $d_1$ being the $\ell_2$ and $\ell_\infty$ norms, respectively, this lemma allows us to replace the upper bound by an expression that only involves the Gaussian width.
 
\begin{lem}[Supremum of process with sub-exponential tails in terms of Gaussian width]\label{lem:Tal_modify}
Let $X_\w$ be a zero-mean symmetric random process in $\R^n$ that satisfies the following three properties.
\begin{enumerate}
\item One of the following holds. 

 Either, for all $\w\in\R^n$, 
\begin{align*}
&\Pr(|X_\w|\geq t) \leq \nn \\
&~~~~~2\exp\Big[-c\min\big\{ \frac{t^2}{K_2^2\|\w\|_2^2}~,~\frac{t}{K_1\|\w\|_\infty} \big\}\Big],
\end{align*}

 Or, for all $\Tc\subset\R^n$,
\begin{align*}
\E\sup_{\w \in \Tc}  X_{\w} \leq C\cdot\big(K_1\,\gamma_1(\Tc, \ell_\infty) + K_2\,\gamma_2(\Tc, \ell_2)\big).
\end{align*}

\item $\E\sup_{\|\w\|_1\leq 1}X_\w \leq B$,

\item For any $\Tc_1,\Tc_2\subset\R^n$, 
\begin{align*}
\E\sup_{\substack{\w=\w_1+\w_2 \\ \w_1\in\Tc_1, \w_2\in\Tc_2}}X_\w \leq \E\sup_{\w_1\in\Tc_1} X_{\w_1} + \E\sup_{\w_2\in\Tc_2} X_{\w_2}.
\end{align*}
\end{enumerate}
Then, the following holds for any subset $\Tc\subset\R^n$:
\bea\nn
\E\sup_{\w\in\Tc}X_\w \leq \Big( \inf_{\theta>0}\big\{ C\, (K_2 +K_1\,\theta) + \frac{C'}{\theta}\, B \big\} \Big) \cdot\wg(\Tc). 
\eea
\end{lem}
Note that in the statement of the lemma, the parameters $K_1, K_2, B>0$ may depend on $n$ and the specific process $X_\w$.
\begin{proof}
Fix a subset $\Tc\subset\R^n$ and a number $\theta>0$. Now, consider the decomposition of $\Tc$ in Proposition \ref{prop:T_decom}. Then, 
\bea \nn
\E\sup_{\w\in\Tc}X_\w &\leq \E\sup_{\substack{\w=\w_1+\w_2 \\\w_1\in\Tc_1, \w_2\in\Tc_2}}X_\w \\
&\overset{(i)}{\leq} \E\sup_{\w_1\in\Tc_1} X_{\w_1} + \E\sup_{\w_2\in\Tc_2} X_{\w_2}\nn\\
&\overset{(ii)}{\leq} C_1 S(K_2+K_1\theta) + \frac{C_2S}{\theta}\cdot\E\sup_{\|\w\|_1\leq 1} X_{\w}\nn \\
&\overset{(iii)}{\leq} C_1 S(K_2+K_1\theta) + \frac{C_2S}{\theta}\cdot B\nn,
\eea
where, (i) follows from property 3 of the lemma; (ii) follows by a combination of property 1, Proposition \ref{prop:Tal_Bern} and  Proposition \ref{prop:T_decom}; and, (iii) follows from property 2. 
Since this holds for all $\theta>0$, this completes the proof.
\end{proof}

